Opportunities and Security Risks of Technical Leverage: A Replication Study on the NPM Ecosystem

To comply with high productivity demands, software developers reuse free open-source software (FOSS) code to avoid reinventing the wheel when incorporating software features. The reliance on FOSS reuse has been shown to improve productivity and the quality of delivered software; however, reusing FOSS comes at the risk of exposing software projects to public vulnerabilities. Massacci and Pashchenko have explored this trade-off in the Java ecosystem through the lens of technical leverage: the ratio of code borrowed from FOSS over the code developed by project maintainers. In this paper, we replicate the work of Massacci and Pashchenko and we expand the analysis to include level-1 transitive dependencies to study technical leverage in the fastest-growing NPM ecosystem. We investigated 14,042 NPM library releases and found that both opportunities and risks of technical leverage are magnified in the NPM ecosystem. Small-medium libraries leverage 2.5x more code from FOSS than their code, while large libraries leverage only 3\% of FOSS code in their projects. Our models indicate that technical leverage shortens the release cycle for small-medium libraries. However, the risk of vulnerability exposure is 4-7x higher for libraries with high technical leverage. We also expanded our replication study to include the first level of transitive dependencies, and show that the results still hold, albeit with significant changes in the magnitude of both opportunities and risks of technical leverage. Our results indicate the extremes of opportunities and risks in NPM, where high technical leverage enables fast releases but comes at the cost of security risks.

==> EMSE_revision.tex <==
\section{EMSE Revision}

\begin{figure}
\centering

\includegraphics[width=\linewidth]{images/use_the_log_regression.pdf}
\caption{xxx}
\label{log_reg}
\end{figure}

==> discussion.tex <==
% \section{Discussion}
% \label{sec:discussion}

% In this section, we discuss some interpretations of our main results and how they impact the software development community.

% \textbf{Popular NPM libraries have lower technical leverage than popular Maven libraries.} 
% In RQ1, we showed that, on median, NPM libraries (2.5x) tend to leverage less code from dependencies than Maven libraries (4.0x). 
% This was counter-intuitive as previous studies have pointed out that NPM projects tend to depend on more dependencies than ecosystems like Maven~\cite{Bogart:21:PracticesPolicies}. 
% While more investigation is needed to understand the reasons why popular NPM packages tend to leverage less from dependencies, one major culprit is the size of libraries in both ecosystems. 
% \diego{To continue...}


% \textbf{Benefits of leveraging dependencies appears more evident in the NPM ecosystem.}



% Risk of 


% \diego{Ahmad wrote this recently. I still need to go over and do my pass. Emad, if you could help us bring some points since you are reading the paper with a fresh mind ;). }
% Our findings in Section~\ref{study_result} show that small-medium libraries have higher direct technical leverage than large libraries in the NPM ecosystem. In fact, our results match the ones in the Maven ecosystem, as shown in the original study. Nevertheless, we find that the NPM libraries considerably have a low direct technical (2.5) leverage than Maven libraries (14.6), as discussed in RQ1. A similar observation is related to the risks. Our results show that high technical leverage leads to more vulnerability exposure in NPM than in Maven, as shown in RQ2. One possible reason for these discrepancies is that the Maven ecosystem is more mature than NPM. Thus, there are more stable, secure, and popular libraries among Java developers, encouraging them to use those libraries in their code. Further studies are required to investigate in detail the centrality~\ahmad{cite Suhaib} of the dependent packages, whether specific packages are used more than others in both Maven and NPM ecosystems to understand libraries usage trends in these ecosystems.

% Although we had similar observations about technical leverage for small-medium and large libraries in Maven and NPM ecosystem, we find that the impact of technical leverage on the release cycle is different. In other words, shipping four times the code in NPM increases the release speed by one day. However, in the Maven ecosystem, it increases the release cycle by 2-6 days. Our results provide insights to NPM developers about the opportunities and risks of using third-party code. Moreover, the findings show that the opportunities and risks might differ across different ecosystems. Therefore, we plan (and encourage others) to replicate our study on other ecosystems such as PyPI and CRAN.

==> tables/L1_stat.tex <==
\begin{tabular}{lrrrrr}

\toprule
\textbf{\# Dependencies} & 
\textbf{Mean} & 
\textbf{Q25\%} &  
\textbf{Median}& 
\textbf{Q75\%} & 
\textbf{Max}\\ 

\midrule
Direct & 7 & 1 & 3 & 9 & 83 \\

Transitive (level-1) & 16 &
 0 &
4&
 19&
320

 \bottomrule
 \end{tabular}

==> tables/contingency_table_L1.tex <==
\begin{tabular}{cccccc}
\toprule
\multicolumn{3}{c}{\textbf{Small-medium libraries}}&
\multicolumn{3}{c}{\textbf{Large libraries}}&

    &  \textbf{\#Vuln}&  \textbf{\#Not vuln} &
    & \textbf{\#Vuln}&  \textbf{\#Not vuln}&
  \midrule
\textbf{\(\lambda\) $>$ 7.75} &  4033& 1011 &\textbf{\(\lambda\) $>$ 0.06} & 1582& 319\\

\textbf{\(\lambda\) $\leq$ 7.75}  &  1456 & 3588 &\textbf{\(\lambda\)  $\leq$ 0.06} & 390& 1617\\
\midrule
\textbf{OR} & 6.7\threeStars & & \textbf{OR} & 20.6\threeStars & \\

\bottomrule
 \end{tabular}
\footnotesize
\begin{flushleft}
\oneStar$p < 0.05$, \twoStars $p < 0.01$, \threeStars$p < 0.001$  \\
\end{flushleft}

==> tables/desc_stats_bkp.tex <==
\begin{tabular}{l|r|r|r|r|r|r|r}
\hline
\textbf{Item} & \textbf{mean} & \textbf{std} & \textbf{min} & \textbf{Q25\%} &  \textbf{median}& \textbf{Q75\%} & \textbf{max}\\ \hline           
 \# versions per lib &100 &94 &9 &39&67&122& 432 \\ \hline
 \# direct deps &7&10&0&1&3&9& 83 \\ \hline
 L\textsubscript{own}(LoC) &7566&11753&10&470&1856&10050&59994 
 \\ \hline
 L\textsubscript{dep}(LoC) &14521&44074&0&232& 2083& 16722&715849\\ \hline

 release interval (days)&23&61&0&1&6&18&1716 \\ \hline
 \end{tabular}

==> tables/desc_stats_vul.tex <==
\begin{tabular}{lrrrrrrr}
\toprule

\textbf{Item} & \textbf{Mean}& \textbf{Min} & \textbf{Q25\%} &  \textbf{Median}& \textbf{Q75\%} & \textbf{Max}\\ 
\midrule
 \# Vulns/own &
 0.3&
 %1.1&
 0&
 0&
 0&
 0&
 9 \\
 \# Vulns/dep &
 2.1&
 %4.2&
 0&
 0&
 0&
 2&
 35 \\
 
 \bottomrule
 \end{tabular}

==> tables/nyc_1_1_8.tex <==
\begin{tabular}{lrrrr}

\toprule
\textbf{Direct Dependencies} &
\multicolumn{4}{c}{\textbf{Transitive Dependencies
}} 
& 
&
\textbf{level-1} &
\textbf{level-2} & 
\textbf{level-3} &  
\textbf{level-4} \\
\midrule
Istanbul & 14 & +17 & +9 & +3  \\
rimraf   & 1 & +6  & +4 & +2 \\
yargs    & 4 & +4 & +4  \\
strip-bom & 2 & & &   \\
mkdirp  &1  & & &   \\
lodash &  & & &  \\

 \bottomrule
 \textbf{sum (71)} &22 &+27&+17&+5 \\
 \hline
 \end{tabular}

==> transitive_deps.tex <==
 \section{The impact of transitive dependencies on the opportunities and risks of the technical leverage }\label{level_one_transitive}
\par

\noindent
\textbf{Motivation.}
So far, our study has focused on assessing the opportunities and risks related to direct dependencies, modelled through the lens of direct technical debt. 
% of a project, which include only direct dependencies.
Direct dependencies are, however, only a small share of the total dependencies of a project. 
As libraries also reuse other libraries code, transitive dependencies quickly become the vast majority of dependencies in a project~\cite{latendresse2022not, prana2021out, decan2017empirical}. 

\haya{Previous researches have shown that transitive dependencies account for a significant portion of dependencies in JavaScript projects. One study estimated that the average number of transitive dependencies in a JavaScript project, when analyzing about 5 million
releases, was 80 (as of 2018) \cite{zimmermann2019small}. Another studies found that half of the npm packages analyzed (317,159 packages, up to 2016) had at least 22 transitive dependencies and a quarter of them had at least 95~\cite{decan2017empirical}, and often packaged to the production package of JavaScript applications ~\cite{latendresse2022not}, where the risks of vulnerabilities are potentially harmful. The importance of
transitive dependencies motivated us to extend the study to evaluate the opportunities and risks of
technical leverage and contrast these findings with direct technical dependency. In this section,
we explore how the benefits and downsides of technical leverage are affected when transitive
dependencies are included.}

Past studies have indicated that transitive dependencies represent in median \diego{X\%} of dependencies of JavaScript projects~\cite{decan2017empirical}, and often packaged to the production package of JavaScript applications~\cite{latendresse2022not}, where the risks of vulnerabilities are potentially harmful.  
The importance of transitive dependencies motivated us to extend the study to evaluate the opportunities and risks of technical leverage and contrast these findings with the direct technical dependency. 
In this section, we explore how the benefits and downsides of technical leverage are affected when transitive dependencies are included.
\\

% In the work of \citet {decan2017empirical}, an analysis of about 317,159 NPM packages showed that about half of the packages had at least 22 transitive dependencies, and a quarter had at least 95 transitive dependencies. A recent empirical study on 100 JavaScript projects by \citet{latendresse2022not}, showed that the majority of production dependencies (51.8\%) are transitive dependencies. 

% \diego{Here we should cite some works (including Jasmine's) to say transitive dependencies are the majority.}

% Looking at the direct dependencies only, the results reveal that the direct technical leverage speeds up software releases but bears a higher risk of exposure to public vulnerabilities. 



% This prompted us to involve transitive dependencies in our analysis for further new investigation.
%The results show in-line findings in comparison to including only direct dependencies, but with a noticeable change in the magnitude of both benefits and downsides.%
% \diego{I would only say this at the end. }

% To obtain deep insights~\diego{deep insights?}, 

\noindent
\textbf{Methodology.}

A comparable study with 14,042 library releases, including all transitive dependencies is too computationally expensive to be practical.
At each library release, we need to compute the size and vulnerabilities of all dependencies. 
Given the exponential growth of transitive dependencies, the median number of dependencies (direct and level one transitive dependencies) on the releases of our dataset can reach up to \diego{XXXX} \haya{7}.
\diego{We need some numbers here to give an idea. Haya gave some numbers of the level 1, but can we estimate how many libraries we would need to compute for a single release in average?}

\begin{table}[]
    \caption{The growth of transitive dependencies for nyc@1.1.8 release.}
    \centering
    \input{tables/nyc_1_1_8.tex}
   
    \label{tab:trans_all}
\end{table} 

\begin{table}[]
 \caption{Comparison of statistics between direct dependencies and level-1 transitive dependencies of 14,042 library releases.}
    \centering
    \input{tables/L1_stat.tex}
    \label{tab:L1_stat}
\end{table}
\haya{Let's now delve into a specific example to further explain the number of libraries that need to be considered for a single release. The release nyc@1.1.8, which is a command line tool for instrumenting code with Istanbul coverage, has 6 direct dependencies and 71 transitive dependencies. Table \ref{tab:trans_all} shows that nyc@1.1.8 release has 22 level-1 transitive dependencies, and if we count for all levels of transitive dependencies, we need to add extra 49 transitive dependencies (more than the double of level-1). This highlights that including all transitive dependencies is impractical due to the high computational cost involved. }

\diego{We could also talk about the paper "On the Effect of Transitivity and Granularity on Vulnerability Propagation in the Maven Ecosystem" which will be presented at SANER. In this paper, they say that up to the level 1 or 2 you already cover most of vulnerabilities (I have to double-check again).} 
\haya{Moreover, according to a recent study \cite{mir2023effect}, packages that have three levels of dependencies, which correspond to level-2 transitive dependencies in our study, were found to have a median of 24 direct and transitive dependencies and were able to cover most of the 94\% vulnerabilities. This could potentially lead to a substantial savings in computation time.}

To make this analysis cost-effective, we opted to analyze the opportunities and risks of technical leverage, considering the level 1 transitive dependency. 
We define a level 1 transitive dependency as any dependency with depth = 2 in a dependency graph, as dependencies with depth = 1 indicate direct dependencies. 
Even considering only level 1 transitive dependencies, our analysis had to analyze a total of \diego{X} \haya {320,253} library releases, as the original set of 14,042 releases have in median 4 other dependencies. 
\diego{Haya, can we compute the exact number? Making the account only on the Q75 is an overestimation (the majority has less than 19 transitive dependencies). }
\haya{320,253=223,021 (L1)+ 97,232 (dir)}




% It is worthy mention that we limit our analysis to include only level 1 transitive dependencies because it is computationally expensive to include all levels of transitive dependencies for 142 packages (14,042 releases). We will show the cost of computation on transitive dependencies of level 1 next.
% The statistical analysis shown in Table \ref{tab:L1_stat} indicates that about 75\% of our sample has 19 transitive dependencies, and some versions reach a maximum of 320 transitive dependencies. This will result in applying the iterative process on about 192,000 releases \haya{ (i.e., 19 (\# transitive dep.) * 0.75 (third quartile) *14,042 (sample size)}, if we consider the count of transitive dependencies in the third quartile . 


% To determine the effect of including transitive dependencies in our analysis, 

% The dependency graph shows which packages the project depends on and how those packages, in turn, depend on other packages. For example, if a package X depends on package A, which depends on package B and package C, then A is a direct dependency with level 0 (depth=1), and B and C are transitive dependencies with level 1 (depth=2).
% ~\diego{We need to better define what first level means}.




We include parallelization to accelerate the analyses of transitive dependencies through  \textsc{concurrent.futures} module, which provides a high-level interface for asynchronously executing.
We divided the original dataset into 14 samples each with 1000 releases, then we apply the computation on each sample using maximum workers equal to the number of processes on our machine (in our case they are 4 processes) as shown on listing \ref {threading}. Considering that we conducted our analysis on a PC running windows 10 Pro,  64-bit operating system with 11th Gen Intel(R) Core(TM) i5-1135G7, 2.42 GHz and 8 GB RAM memory.


\begin{minipage}{\linewidth} 
\begin{lstlisting} [caption={Snippet code of multithreading computation to resolve transitive dependencies.},label={threading},language=Python] 
num_procs = psutil.cpu_count(logical=False)
splitted_df = np.array_split(df, num_procs)
with concurrent.futures.ProcessPoolExecutor(max_workers=num_procs) as executor:
    results = [ executor.submit(resolve_trans_deps,df=df) for df in splitted_df ]
        .....
\end{lstlisting}
\end{minipage}

\diego{I loved the details - I am a performance guy by formation and I asked for more details originally  - but I think this is too detailed for an EMSE paper. Thank you, Haya! We should just say, we analyzed X dependencies, used parallelization and this overall took 6 full days of computing power. Ahmad, I will leave to you to shrink this part.}
As an initial step, the computations cost us about 0.5-1 minute/package releases to extract level 1 transitive dependencies, this counts for 1.2-2.37 hours ( 0.5-1 minute * 142 packages), considering 75\% of our sample have 9 direct dependency and can reach up to 83 direct dependency, this is computationally the cheapest step.
The most expensive steps are related to resolving transitive dependencies and computing the size of release (LOC). Next step (resolving transitive dependencies) costs about 5,55-7,22 hours/1000 release, if we consider the lower bound (5,55 hours), this costs about 78 hours (i.e., 5.55*14,042/1,000) (more than 3 full day of computation). Adding to the above mentioned cost, the computation of the release size (LOC) costs about 4.5 hours/1000 release (2.6 full day of computation). In total, we need more than 5 days for just computing level 1 transitive dependencies.
This implies that including all transitive dependencies can be particularly challenging because they can create exponential complexity in terms of computation. 
\\


\noindent
\textbf{Results:}
\diego{We need to organize the results a bit better. Ahmad, can you take a crack at it and I do a pass afterwards? Maybe we could use subsections for each RQ or just give more context before diving into the results...}
We discuss the results of our extended analysis by reporting on the impact of considering level-1 transitive dependencies on the opportunities and risks of direct technical leverage.

For \textbf{RQ1}, which studies if there is a difference in direct technical leverage between small-medium and large libraries, we find that small-medium library releases leverage, on median, 7.75 times of their own code in FOSS, when including transitive dependencies, in comparison to 2.5 times when library releases consider only the direct dependencies. A gradual increase in magnitude is observed for large library releases, where the median leverage increased from 3\% (i.e. when leverage depends on direct dependencies only), to  6\% when including transitive dependencies. Figure \ref{direct_lev} and Figure \ref{trans_lev} show that small-medium libraries ship other people’s code more than large libraries, with an increase in magnitude when the technical leverage includes the transitive dependencies in its computation. 

\begin{figure*}
\includegraphics[width=\linewidth]{images/distribution_leverage_own_size.pdf}
\caption{The technical leverage of 14,042 library releases per library size in LOC.}
\label{trans_lev}
\end{figure*}

\begin{figure}
% \includegraphics[width=\linewidth]{images/SourceOfVul.pdf}
\includegraphics[width=.7\linewidth]{images/source_vulnerabilities_with_L1.pdf}
\caption{Count of all vulnerabilities reported in small-medium and large library releases per vulnerability source and technical leverage. Note that the y axis is in log-scale.}
\label{source_vul_trans}
\end{figure}


On the other hand, we investigate the influence of transitive dependencies on the \textbf{RQ2} results, this research question explores the effect of direct technical leverage on the release interval between library releases. Return back to the results of RQ2 in \ref{rq2}, the model suggests that a 4 times increase in the direct technical leverage ($\lambda_{dir}$) of all
libraries affects the predicted mean release interval cycle in one day.
On the other hand, we observe that when including transitive dependencies, small-medium libraries still benefit from technical leverage. On other words, libraries that leverage more FOSS code seems to release faster, but with a slight less magnitude of speed. However, the technical leverage has no influence on the large libraries release cycle with and without including transitive dependencies.


Previous studies \cite{kula2018developers, pashchenko2018vulnerable} highlight that transitive dependencies inflate the problem of vulnerabilities, for that, we resort to check the impact of technical leverage  (including transitive dependencies) on the health of library releases, on the aim to find the differences between new observed results and the results of \textbf{RQ3} elaborated in \ref{rq3}, where the direct technical leverage ($\lambda_{dir}$) increases the security risks. The extended analysis (including transitive dependencies) shows that technical leverage increases the magnitude of security risks for both small-medium and large libraries. The risk of having vulnerabilities reported increases 6.7-folds \haya{This is OR ratio.. included in a tbel 5} in small-medium libraries that rely on high technical leverage in comparison to 4-folds when they depend on high direct technical leverage ($\lambda_{dir}$)  as shown previously in  Table \ref{table_contengency}. Moreover, large libraries that rely on high technical leverage have about 21 times more risk of being affected by reported vulnerabilities in comparison to 7 times  when they rely on high direct technical leverage ($\lambda_{dir}$). 
Additionally, the extended analysis shows that dependencies are the primary source of vulnerability for both small-medium and large library releases as illustrated in Figure \ref{source_vul} (direct dependencies) and Figure \ref{source_vul_trans} (transitive dependencies), where including transitive dependencies in small-medium size libraries bloats the problem of vulnerabilities, except for large libraries with low technical leverage. The analysis of our dataset, including transitive dependencies, shows that the number of all security vulnerabilities reported in small- medium library releases, increases by 2.6 times (48,848/18,789) and about 1.9 times for large libraries, considering the high technical leverage. 
As we expected, we found that small and medium libraries with technical leverage above 7.75 have a higher chance of encountering more vulnerabilities , 5 or more vulnerabilities, as shown in Figure \ref{vul_max_small_trans}, in addition to an increase in the maximum number of vulnerabilities from 35 to 74, as shown in Figures \ref{vul_max_small} and \ref{vul_max_small_trans} respectively. 

\begin{figure}[tb]
\includegraphics[width=\linewidth]{images/vul_vs_leverage_small_trans.pdf}
\caption{Technical leverage per library vs Number of vulnerabilities for small-medium library releases.}
\label{vul_max_small_trans}
\end{figure}

% \begin{figure}[tb]
% \includegraphics[width=.9\linewidth]{images/vul_vs_leverage_large_trans.pdf}
% \caption{Technical leverage per library vs Number of vulnerabilities for large library releases.}
% \label{vul_max_large_trans}
% \end{figure}

\haya{To summarize, the results, when including transitive dependencies (level 1), show in-line findings in comparison to including only direct dependencies, but with a noticeable change in the magnitude of both benefits and downsides.}
